Loeb Extension and Loeb Equivalence

In Keisler and Sun (2004), the authors raise several open problems on Loeb equivalences between various internal probability spaces. We provide counter-examples for the first two open problems. Moreover, we reduce the third open problem to the following question: Is the internal algebra generated by the union of two Loeb equivalent internal algebras a subset of the Loeb extension of any one of the internal algebra?

==> loeb equivalence arxiv/bib.tex <==
\usepackage[%
    minnames=1,maxnames=99,maxcitenames=3,
    style=alphabetic,
    doi=false,url=false,
    firstinits=true,hyperref,natbib,backend=bibtex]{biblatex}
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}}
\bibliography{biblio}



==> loeb equivalence arxiv/commenting.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% EDITING HELPER FUNCTIONS  %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% NA: needs attention (rough writing whose correctness needs to be verified)
%% TBD: instructions for how to fix a gap ("Describe the propagation by ...")
%% PROBLEM: bug or missing crucial bit 

%% use \fXXX versions of these macros to put additional explanation into a footnote.  
%% The idea is that we don't want to interrupt the flow of the paper or make it 
%% impossible to read because there are a bunch of comments.

%% NA's (and TBDs, those less crucially) should be written so 
%% that they flow with the text.

\definecolor{WowColor}{rgb}{.75,0,.75}
\definecolor{SubtleColor}{rgb}{0,0,.50}

% inline
\newcommand{\NA}[1]{\textcolor{red}{ {\tiny \bf ($\star$)} #1}}
\newcommand{\LATER}[1]{\textcolor{SubtleColor}{ {\tiny \bf ($\dagger$)} #1}}
\newcommand{\TBD}[1]{\textcolor{SubtleColor}{ {\tiny \bf (!)} #1}}
\newcommand{\PROBLEM}[1]{\textcolor{WowColor}{ {\bf (!!)} {\bf #1}}}

% as margin notes

\newcounter{margincounter}
\newcommand{\displaycounter}{{\arabic{margincounter}}}
\newcommand{\incdisplaycounter}{{\stepcounter{margincounter}\arabic{margincounter}}}

\newcommand{\fTBD}[1]{\textcolor{SubtleColor}{$\,^{(\incdisplaycounter)}$}\marginpar{\tiny\textcolor{SubtleColor}{ {\tiny $(\displaycounter)$} #1}}}
\newcommand{\fPROBLEM}[1]{\textcolor{WowColor}{$\,^{((\incdisplaycounter))}$}\marginpar{\tiny\textcolor{WowColor}{ {\bf $\mathbf{((\displaycounter))}$} {\bf #1}}}}
\newcommand{\fLATER}[1]{\textcolor{SubtleColor}{$\,^{(\incdisplaycounter\dagger)}$}\marginpar{\tiny\textcolor{SubtleColor}{ {\tiny $(\displaycounter\dagger)$} #1}}}


==> loeb equivalence arxiv/defs.tex <==
% !TEX root =  completeclass.tex

\def\[#1\]{\begin{align}#1\end{align}}
\def\*[#1\]{\begin{align*}#1\end{align*}}

\newcommand{\defas}{\vcentcolon=}  % requires mathtools package
%\newcommand{\defas}{\equiv}

\newcommand{\argdot}{\cdot}

%% such that
\newcommand{\st}{\,:\,}

%% for writing  A | X ~ P(X) statements
\newcommand{\dist}{\ \sim\ }
\newcommand{\given}{\mid}
\newcommand{\distiid}{\overset{iid}{\dist}}
\newcommand{\distind}{\overset{ind}{\dist}}


\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Rationals}{\mathbb{Q}}
\newcommand{\Reals}{\mathbb{R}}
%\newcommand{\BorelSets}{\mathcal{B}}
\newcommand{\Nats}{\mathbb{N}}
\newcommand{\Ints}{\mathbb{Z}}
\newcommand{\NNInts}{\Ints_+}
\newcommand{\NNExtInts}{\overline{\Ints}_+}
\newcommand{\Cantor}{\2^\mathbb{N}}
\newcommand{\NNReals}{\Reals_{\ge 0}}
\newcommand{\PosReals}{\Reals_{> 0}}

\newcommand{\as}{\textrm{a.s.}}

\newcommand{\epi}{\textrm{epi}}
\newcommand{\intr}{\textrm{int}}
\newcommand{\conv}{\textrm{conv}}
\newcommand{\cone}{\textrm{cone}}
\newcommand{\aff}{\textrm{aff}}
\newcommand{\dom}{\textrm{dom}}
\newcommand{\cl}{\textrm{cl}}
\newcommand{\ri}{\textrm{ri}}
\newcommand{\grad}{\nabla}
\newcommand{\imp}{\Rightarrow}
\newcommand{\downto}{\!\downarrow\!}
\newcommand{\upto}{\!\uparrow\!}

%\newcommand{\ind}{\perp\!\!\!\perp}
\newcommand{\ind}{\mathrel{\perp\mkern-9mu\perp}}
%\newcommand\ind{\protect\mathpalette{\protect\independenT}{\perp}}
%\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern5mu{#1#2}}}

\newcommand{\AND}{\wedge}
\newcommand{\OR}{\vee}
\newcommand{\NOT}{\neg}

\newcommand{\dee}{\mathrm{d}}

\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\sign}{sign}

\DeclareMathOperator*{\newlim}{\mathrm{lim}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newmin}{\mathrm{min}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newmax}{\mathrm{max}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newinf}{\mathrm{inf}\vphantom{\mathrm{infsup}}}
\DeclareMathOperator*{\newsup}{\mathrm{sup}\vphantom{\mathrm{infsup}}}
\renewcommand{\lim}{\newlim}
\renewcommand{\min}{\newmin}
\renewcommand{\max}{\newmax}
\renewcommand{\inf}{\newinf}
\renewcommand{\sup}{\newsup}

%\newcommand{\card}[1]{\#(#1)}


\renewcommand{\Pr}{\mathbb{P}}
\def\EE{\mathbb{E}}
\DeclareMathOperator*{\var}{var}

%% definition
\newcommand{\defn}[1]{\emph{#1}}

\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceiling}[1]{\lceil #1 \rceil}

\def\bone{\mathbf{1}}
\def\Ind{\bone}

\newcommand{\cF}{\mathcal F}
\newcommand{\cG}{\mathcal G}

\DeclareMathOperator*{\Beta}{Beta}
\DeclareMathOperator*{\Bernoulli}{Bernoulli}
\DeclareMathOperator*{\PP}{PP}
\DeclareMathOperator*{\Poisson}{Poisson}
\newcommand{\Uniform}{\textrm U (0,1)}

\newcommand{\equaldist}{\overset{d}{=}}
\newcommand{\inv}{^{-1}}

\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\event}[1]{\left \lbrace #1 \right \rbrace}
\newcommand{\tuple}[1]{\langle #1 \rangle}


\newcommand{\bspace}{\Omega}
\newcommand{\bsa}{\mathcal A}
\newcommand{\borelspace}{(\bspace,\bsa)}


\newcommand{\card}[1]{\##1}
%\newcommand{\as}{\textrm{a.s.}}
\newcommand{\iid}{i.i.d.}

%% for writing down stochastic processes
\newcommand{\gprocess}[2]{(#1)_{#2}}
\newcommand{\nprocess}[3]{\gprocess{#1_{#3}}{#3 \in #2}}
\newcommand{\process}[2]{\nprocess{#1}{#2}n}


%% not in love with these...
\newcommand{\of}[1]{\left ( #1 \right )}
\newcommand{\oof}[1]{( #1 )}
\newcommand{\ooof}[1]{\bigl ( #1 \bigr )}
\newcommand{\oooof}[1]{\Bigl ( #1 \Bigr )}
\newcommand{\ooooof}[1]{\biggl ( #1 \biggr )}
\newcommand{\oooooof}[1]{\Biggl ( #1 \Biggr )}

\newcommand{\oF}[1]{\left [ #1 \right ]}
\newcommand{\ooF}[1]{[ #1 ]}
\newcommand{\oooF}[1]{\bigl [ #1 \bigr ]}
\newcommand{\ooooF}[1]{\Bigl [ #1 \Bigr ]}
\newcommand{\oooooF}[1]{\biggl [ #1 \biggr ]}
\newcommand{\ooooooF}[1]{\Biggl [ #1 \Biggr ]}

\newcommand{\Of}[1]{\left \{ #1 \right \}}
\newcommand{\Oof}[1]{\{ #1 \}}
\newcommand{\Ooof}[1]{\bigl \{ #1 \bigr \}}
\newcommand{\Oooof}[1]{\Bigl \{ #1 \Bigr \}}
\newcommand{\Ooooof}[1]{\biggl \{ #1 \biggr \}}
\newcommand{\Oooooof}[1]{\Biggl \{ #1 \Biggr \}}


%%%%% add definitions here


\DeclareMathOperator{\cf}{cf}

\newcommand{\lind}{Lindel\"{o}f }
\newcommand{\prepro}[2]{r^{-1}_{#1} r_{#1} (#2)}
\newcommand{\preprop}[2]{p^{-1}_{#1} p_{#1} (#2)}
\newcommand{\preprorho}[2]{\rho^{-1}_{#1} \rho_{#1} (#2)}
\newcommand{\preprov}[2]{\varpi^{-1}_{#1} \varpi_{#1} (#2)}
\newcommand{\precs}[1]{{| \mathsf{#1} \rangle }}

\newcommand{\BorelSets}[1]{\mathcal{B}[#1]}
\newcommand{\NSE}[1]{{^{*}#1}}
\newcommand{\ST}{\mathsf{st}}
\newcommand{\SP}[1]{{^{\circ}#1}}
\newcommand{\MFuncs}{\mathcal{M}}

%\newtheorem*{EPrinciple}{Extension}
%\newtheorem*{TPrinciple}{Transfer}
%\newtheorem*{SPrinciple}{Saturation}

\newcommand{\Procs}{\cQ}


\newcommand{\InternalSubsets}[1]{\mathcal I[#1]}


\newcommand{\XX}{X}
\newcommand{\XXSA}{\mathcal X}
%\newcommand{\Theta}{\Theta}
\newcommand{\ThetaSA}{\mathcal T}
\newcommand{\Actions}{\cA}
\newcommand{\AS}{A}
\newcommand{\ASSA}{\mathcal A}


\newcommand{\PowerSet}{\mathscr{P}}
\newcommand{\HReals}{\NSE{\Reals}}

\newcommand{\Model}{P}
\newcommand{\hfModel}{P'}
\newcommand{\Loss}{\ell}
\newcommand{\hfLoss}{L}
\newcommand{\NS}[1]{\mathrm{NS}(#1)}
\newcommand{\XY}{XY}
\newcommand{\Risk}{r}
\newcommand{\hfRisk}{R}

\newcommand{\cS}{\mathcal{S}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cE}{\mathbb{E}}

%\newcommand{\IFuncs}[2]{\mathrm{I}({#1}^{#2})}
\newcommand{\IFuncs}[2]{\mathrm{I}({#1}^{#2})}

\newcommand{\FiniteSubsets}[1]{{#1}^{[< \infty]}}
\newcommand{\hfRiskSpace}{\IFuncs {\HReals} {K_{\Theta}}}

\newcommand{\hyperapprox}{(S_{X},B_{X},S_{\Theta},B_{\Theta},(\hfModel)_{t},\hfLoss)}
%\newtheorem{problem}{Problem}

\newcommand{\vzero}{\mathbf{0}}
\newtheorem{open problem}{Open Problem}

\newcommand{\Loeb}[1]{\overline{#1}}
\newcommand{\LoebAlgebra}[2]{\overline{#1}_{#2}}

\newcommand{\NICE}[2]{C[#1,#2]}
\newcommand{\iA}[1]{\mathcal A[#1]}


%\newcommand{\Measures}{\mathcal{M}}
%\newcommand{\ProbMeasures}{\mathcal{M}_1}
\newcommand{\ProbMeasures}[1]{\mathcal{M}_1(#1)}

%\newcommand{\SF}{\tilde\cD}
\newcommand{\IEs}{\FiniteRiskEstimators}
%\newcommand{\IREs}{\cD^{*}}
%\newcommand{\IELs}{\cD^L}
%\newcommand{\DSF}{\SF^{[*]}}
\newcommand{\IPMs}[1]{\mathcal P(#1)}

\newcommand{\gX}{X}
\newcommand{\gY}{Y}

\newcommand{\Tail}[2]{\NSE{#1} \setminus \bigcup B_{#2}}



\newcommand{\interior}[1]{%
  {\kern0pt#1}^{\mathrm{o}}%
}

\newcommand{\Language}{\mathcal L}

\newcommand{\FRRE}{\mathcal D}
\newcommand{\FRREFS}{\FRRE_{0,FC}}
\newcommand{\sFRREFS}{\NSE{\!\FRREFS}}
\newcommand{\FiniteRiskEstimators}{\FRRE_0}
\newcommand{\refproof}[1]{See \cref{#1} for \IfSubStr{#1}{,}{proofs}{a proof}. }
\newcommand{\Rational}{\mathbb{Q}}
\newcommand{\Idc}[1]{\mathbb{I}_{#1}}

\newcommand{\sconv}{\NSE{\!\conv}}

\newcommand{\TTheta}{T_{\Theta}}
\newcommand{\ttheta}{t}
\newcommand{\STK}{J_{\Theta}}
\newcommand{\DRiskSpace}{\IFuncs{\HReals}{\STK}}

\newcommand{\ExtFiniteRiskEstimators}{{\FiniteRiskEstimators}^{\!\!\!*}}
\newcommand{\ExtFRRE}{\FRRE^{*}}

\newcommand{\FSE}{(\ExtFiniteRiskEstimators)_{FC}}
%\newcommand{\FSE}{\FRRE_{0,FC}^{*}}
\newcommand{\FSERS}{\mathcal S^{\FSE}}

\newcommand{\FRREFSRS}{\mathcal S^{\sFRREFS}}

\newcommand{\sFiniteRiskEstimators}{\NSE{\!\FiniteRiskEstimators}}
\newcommand{\sFRRE}{\NSE{\!\FRRE}}

\newcommand{\sdelta}{\NSE{\!\delta}}
\newcommand{\sRisk}{\NSE{\!\Risk}}

\newcommand{\EEst}[1]{\mathbb{E}(#1)}

\newcommand{\IP}[2]{\langle #1, #2\rangle}

\newcommand{\Fincomb}[1]{(#1)_{FC}}
\newcommand{\spEssCompleteSubclass}[1]{$\SP{}$essentially complete subclass of $#1$}
\newcommand{\spCompleteSubclass}[1]{$\SP{}$complete subclass of $#1$}


\newif\iflongform
\longformtrue
%\longformfalse

\iflongform
 \newcommand{\EpsDom}[1]{$#1$-dominated}
 \newcommand{\EpsAdmissible}[2]{$#1$-admissible among $#2$}
 \newcommand{\ExtAdmissible}[1]{extended admissible among $#1$}
 \newcommand{\Admissible}[1]{admissible among $#1$}

 \newcommand{\spDomIn}[2]{$\SP{}$dominated in $#1/#2$}
 \newcommand{\spDom}[1]{$\SP{}$dominated on $#1$}
 \newcommand{\spEpsDomIn}[3]{$#1$-$\SP{}$dominated in $#2/#3$}
 \newcommand{\spEpsDom}[2]{$#1$-$\SP{}$dominated on $#2$}
 \newcommand{\spEpsAdmissibleIn}[4]{$#1$-$\SP{}$admissible in $#2/#3$ among $#4$}
 \newcommand{\spEpsAdmissible}[3]{$#1$-$\SP{}$admissible on $#2$ among $#3$}
 \newcommand{\spExtAdmissible}[2]{$\SP{}$extended admissible on $#1$ among $#2$}
 \newcommand{\spAdmissibleIn}[3]{$\SP{}$admissible in $#1/#2$ among $#3$}
 \newcommand{\spAdmissible}[2]{$\SP{}$admissible on $#1$ among $#2$}
% \newcommand{\spDom}[2]{$\SP{}$dominated in $#1$ over $#2$}
% \newcommand{\spEpsDom}[3]{$#1$-$\SP{}$dominated in $#2$ over $#3$}
% \newcommand{\spEpsAdmissible}[4]{$#1$-$\SP{}$admissible in $#2$ over $#3$ among $#4$}
% \newcommand{\spExtAdmissible}[3]{$\SP{}$extended admissible in $#1$ over $#2$ among $#3$}
% \newcommand{\spAdmissible}[3]{$\SP{}$admissible in $#1$ over $#2$ among $#3$}
\else
 \newcommand{\EpsDom}[1]{$#1$-dominated}
 \newcommand{\EpsAdmissible}[2]{$(#1,#2)$-admissible}
 \newcommand{\ExtAdmissible}[1]{$#1$-extended admissible}
 \newcommand{\Admissible}[1]{$#1$-admissible}

 \newcommand{\spDom}[1]{$#1$-$\SP{}$dominated}
 \newcommand{\spEpsDom}[3]{$(#1,#2,#3)$-$\SP{}$dominated}
 \newcommand{\spEpsAdmissible}[3]{$(#1,#2,#3)$-$\SP{}$admissible}
 \newcommand{\spExtAdmissible}[2]{$(#1,#2)$-$\SP{}$extended admissible}
 \newcommand{\spAdmissible}[2]{$(#1,#2)$-$\SP{}$admissible}
\fi


\newcommand{\GENRS}{\cS^{\cC}}

\newcommand{\RS}[1]{\cS^{#1}}

\newcommand{\Ext}[1]{#1^{*}}
\newcommand{\FC}[1]{(#1)_{FC}}

\newcommand{\FSC}{\cF}

\newcommand{\Normal}[2]{\mathcal N(#1,#2)}
\newcommand{\Identity}{I}
\newcommand{\bx}{\mathbf{x}}


==> loeb equivalence arxiv/headers.tex <==
% !TEX root =  donotcompileme.tex

%\usepackage{amsaddr}
\usepackage[utf8]{inputenc}
\usepackage{amsmath, amssymb,bm, cases, mathtools, thmtools}
\usepackage{verbatim}
\usepackage{graphicx}\graphicspath{{figures/}}
\usepackage{multicol}
\usepackage{tabularx}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{mathrsfs}
\usepackage{url}
\usepackage[normalem]{ulem}
\usepackage{xstring}
\usepackage{enumitem}

%% load locally so we can use biblatex or natbib as needed for journal
\input{bib.tex}

\usepackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=RawSienna]{hyperref}
\usepackage{hypernat}
\usepackage{datetime}

%% change up the fonts for fun.
%\usepackage[OT1]{eulervm}
%\usepackage{palatino}

\DeclareMathAlphabet\EuRoman{U}{eur}{m}{n}
\SetMathAlphabet\EuRoman{bold}{U}{eur}{b}{n}
\newcommand{\eurom}{\EuRoman}

%% hide equation numbers for unreferenced equations
%\mathtoolsset{showonlyrefs}

%% make text prettier
\usepackage{euscript,microtype}
%\DisableLigatures{encoding = *, family = * }

%% nicer way of making \ref'ences to theorems, lemmas, equations, sections, etc.
\usepackage[capitalize]{cleveref}

%% add entries for anything missing.
\crefname{assumption}{Assumption}{Assumptions}
\crefname{claim}{Claim}{Claims}

%% grey out the equation numbers slightly
\makeatletter
\let\reftagform@=\tagform@
\def\tagform@#1{\maketag@@@{\ignorespaces\textcolor{gray}{(#1)}\unskip\@@italiccorr}}
\renewcommand{\eqref}[1]{\textup{\reftagform@{\ref{#1}}}}
\makeatother


%% standard marginalia note
\setlength{\marginparwidth}{1.25in}

% reshape the page to make it wider
%\usepackage[paperwidth=185.7mm,
%      paperheight=241.2mm,
%      textwidth=140mm,
%      textheight=230mm,
%      left=12mm]{geometry}
%\setlength{\marginparwidth}{27mm}

%% Monitor
%\usepackage[paperwidth=8in,paperheight=9in,textwidth=6in, textheight=8in,left=.5in]{geometry}
%\setlength{\marginparwidth}{1.5in}

\input{commenting.tex}

%% theorem styles
\declaretheorem[style=plain,numberwithin=section,name=Theorem]{theorem}
\declaretheorem[style=plain,sibling=theorem,name=Lemma]{lemma}
\declaretheorem[style=plain,sibling=theorem,name=Proposition]{proposition}
\declaretheorem[style=plain,sibling=theorem,name=Corollary]{corollary}
\declaretheorem[style=plain,sibling=theorem,name=Claim]{claim}

\declaretheorem[style=definition,sibling=theorem,name=Definition]{definition}
\declaretheorem[style=definition,name=Assumption]{assumption}
\declaretheorem[style=definition,sibling=theorem,name=Example]{example}
\declaretheorem[style=remark,sibling=theorem,name=Remark]{remark}
%\declaretheorem[style=definition,qed=$\triangleleft$,sibling=theorem,name=Example]{example}
%\declaretheorem[style=remark,qed=$\triangleleft$,sibling=theorem,name=Remark]{remark}
%\declaretheorem[style=definition,qed=$\triangleleft$,sibling=theorem]{fact}


\declaretheorem[style=definition,name=Condition]{conditionINNER}
\newenvironment{condition}[1]
 {\renewcommand{\theconditionINNER}{#1}\conditionINNER}
 {\endconditionINNER}
\crefformat{conditionINNER}{#2(#1)#3}
\crefmultiformat{conditionINNER}
  {(#2#1#3)}
  { and~(#2#1#3)}
  {, (#2#1#3)}
  { and~(#2#1#3)}
\Crefformat{conditionINNER}{Condition~#2(#1)#3}
\Crefmultiformat{conditionINNER}
  {Conditions~(#2#1#3)}
  { and~(#2#1#3)}
  {, (#2#1#3)}
  { and~(#2#1#3)}

%
%\declaretheorem[style=definition,name=Condition]{conditionINNER}
%
%\newenvironment{condition}[1]
% {\renewcommand{\theconditionINNER}{(#1)}\conditionINNER}
% {\endconditionINNER}
%\crefname{conditionINNER}{Condition}{Conditions}
%\crefformat{conditionINNER}{#1}
%\crefmultiformat{conditionINNER}
%  {#2#1#3}
%  { and~#2#1#3}
%  {, #2#1#3}
%  { and~#2#1#3}
%\Crefformat{conditionINNER}{#2#1#3}
%\Crefmultiformat{conditionINNER}
%  {#2#1#3}
%  { and~#2#1#3}
%  {, #2#1#3}
%  { and~#2#1#3}


\declaretheoremstyle[
    spaceabove=-6pt,
    spacebelow=6pt,
    headfont=\normalfont\bfseries,
    bodyfont = \normalfont,
    postheadspace=1em,
    qed=$\square$,
    headpunct={{}}]{myproofstyle}
\declaretheorem[name={}, style=myproofstyle, unnumbered]{appproof}

\numberwithin{equation}{section}
\numberwithin{theorem}{section}

\renewcommand{\appendixname}{}
%\renewcommand{\sectionname}{\S}

%% put ruler down the side for draft, and color it gray
%\usepackage{vruler}
%\setvruler[10pt][1][1][4][1][20pt][20pt][0pt][\textheight]
%\let\orgfillzeros\fillzeros
%\def\fillzeros[#1]#2{%
%  \begingroup
%    \color[rgb]{0.8,0.8,0.8}%
%    \orgfillzeros[{#1}]{#2}%
%  \endgroup
%}

\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{leftidx}

\renewenvironment{quote}
               {\list{}{\rightmargin\leftmargin}%
                \item\relax}
               {\endlist}



==> loeb equivalence arxiv/loebabstract.tex <==
In \citep{loebsun}, the authors raise several open problems on Loeb equivalences between various internal probability spaces. We provide counter-examples for the first two open problems. Moreover, we reduce the third open problem to the following question:  Is the internal algebra generated by the union of two Loeb equivalent internal algebras a subset of the Loeb extension of any one of the internal algebra? 


==> loeb equivalence arxiv/loebeq.tex <==
\section{Introduction}
The Loeb measure construction (\citep{Loeb75}) has provided many fruitful applications in various areas in mathematics such as probability theory (see \citep{andersonisrael}, \citep{nsweak}, \citep{localtime}, \citep{Keisler87}, \citep{stoll}, \citep{brownfrac}, \citep{hylevy}, \citep{Markovpaper}, \citep{anderson2018mixhit} etc), statistical decision theory (see \citep{nsbayes}), potential theory (\citep{loebpotential}), mathematical physics (see \citep{nsphysics}) and mathematical economics (see \citep{robeco}, \citep{ali74}, \citep{nsexchange}, \citep{alir75}, \citep{oligopoly}, \citep{rashid78}, \citep{emmons84}, \citep{strongcore}, \citep{secondwelfare}, \citep{andersonbook}, \citep{lawlarge}, \citep{purestrategy}, \citep{sun99}, \citep{khansun991}, \citep{khansun992}, \citep{rauh07}, \citep{indmatching}, \citep{anderson08}, \citep{xsun16}, \citep{duffie18}, \citep{stochasticmec} etc). \footnote{\citep{robeco}, \citep{ali74}, \citep{nsexchange}, \citep{alir75} and \citep{oligopoly} predated the Loeb measure construction. They relied on a careful analysis of the close relationship between the discrete and measure-theoretic properties of hyperfinite sets that the Loeb measure construction so perfectly captures. The arguments in these papers led, via a Loeb space argument, to a very general and completely elementary argument given in \citep{core1}.} These applications are supported by the development of mathematical infrastructures such as integration theory (see \citep{Loeb75} and \citep{andersonisrael}), representation of measures (see \citep{anderson87} and \citep{stincomb}) and Fubini theorem (see \citep{Keisler87}). \citet{loebsun} made an important contribution to the infrastructure, but left four open problems. We give complete solutions to the first two open problems as well as a partial solution to the third open problem. 

Given an internal probability space $(\Omega, \cF, \mu)$, its Loeb extension is defined to be the countably additive probability space $(\Omega, \Loeb{\cF}, \Loeb{\mu})$, where $\Loeb{\cF}$ consists of all sets $B\subset \Omega$ such that
\[
\sup\{\ST(\mu(A)): B\supset A\in \cF\}=\inf\{\ST(\mu(C)): B\subset C\in \cF\}
\] 
and $\Loeb{\mu}(B)$ is defined to be the above supremum. \citet{loebsun} introduced the following definition to compare two internal probability spaces. 

\begin{definition}\label{defloebext}
Let $\cM=(\Omega, \cF, \mu)$ and $\cN=(\Omega, \cG, \nu)$ be two internal probability spaces. 
We say $\cN$ \textbf{Loeb extends} $\cM$ if $\Loeb{\cG}\supset \Loeb{\cF}$ and $\Loeb{\nu}$ extends $\Loeb{\mu}$ as a function. 
We say $\cN$ is \textbf{Loeb equivalent to} $\cM$ if $\Loeb{\cF}=\Loeb{\cG}$ and $\Loeb{\nu}=\Loeb{\mu}$.  
\end{definition}

If $\cF\subset \cG$ and $\nu$ extends $\mu$ as a function, then it is clear that $\cN$ Loeb extends $\cM$. 
However, as pointed out by \citet{loebsun}, Loeb extensions and Loeb equivalence are much more difficult when it is not assumed that $\cF\subset \cG$. As a result, \citet{loebsun} have left four open problems on Loeb extensions and Loeb equivalences. 
We give complete/partial solutions to the first three open problems, which we list below. We say an internal probability space 
$(\Omega, \cF, \mu)$ is \textbf{hyperfinite} if $\cF$ is hyperfinite (As in \citep{loebsun}, we do not require $\Omega$ to be hyperfinite). 

\begin{question}\label{loebeqq1}
Suppose $\cN$ Loeb extends $\cM$. Must $\cN$ has an internal subspace that is Loeb equivalent to $\cM$? What if $\cM$ is assumed to be hyperfinite? 
\end{question} 

\begin{question}\label{loebeqq2}
Suppose $\cN$ Loeb extends $\cM$ and $\cN$ is hyperfinite. Must $\cM$ be Loeb equivalent to a hyperfinite probability space? 
\end{question}

\begin{question}\label{loebeqq3}
Suppose $\cM=(\Omega, \cF, \mu)$ is Loeb equivalent to $\cN=(\Omega, \cG, \nu)$, and $\cH$ be the internal algebra generated by $\cF\cup \cG$.
Must there be an internal probability measure $P$ on $\cH$ such that $\cM$ is Loeb equivalent to $(\Omega, \cH, P)$? What if $\cM$ and $\cN$ are assumed to be hyperfinite? 
\end{question}


\section{Counter-examples for the First Two Questions}
We start this section by introducing the following theorem which provides a useful characterization of Loeb extension. The first part of the theorem is cited from {\citep[][Lemma.~4.3]{loebsun}}.
\begin{theorem}\label{loebeqlemma}
Let $\cM=(\Omega, \cF, \mu)$ and $\cN=(\Omega, \cG, \nu)$ be two internal probability spaces. 
\begin{itemize}
\item $\cN$ Loeb extends $\cM$ if and only if for every $B\in \cF$ there exists $C\in \cG$ such that $B\subset C$ and $\nu(C)\approx \mu(B)$.

\item $\cN$ Loeb extends $\cM$ if and only if for every $B\in \cF$ there exists $C\in \cG$ such that $C\subset B$ and $\nu(C)\approx \mu(B)$.
\end{itemize}
\end{theorem}
\begin{proof} 
The first statement is cited directly from {\citep[][Lemma.~4.3]{loebsun}}. 
We give a proof of the second statement for completeness.  
Suppose $\cN$ Loeb extends $\cM$ and pick $B\in \cF$. 
Then there exists $C\in \cG$ such that $\Omega\setminus B\subset C$ and $\nu(C)\approx \mu(\Omega\setminus B)$. 
Thus, we have $\Omega\setminus C\subset B$ and $\nu(\Omega\setminus C)\approx \mu(B)$. 
Conversely, for every $B\in \cF$, there exists $C\in \cG$ such that $C\subset \Omega\setminus B$ and $\nu(C)\approx \mu(\Omega\setminus B)$. 
Hence, we have $B\subset \Omega\setminus C$ and $\nu(\Omega\setminus C)\approx \mu(B)$. 
By the first statement, we know that $\cN$ Loeb extends $\cM$. 
\end{proof} 

Suppose $\cN$ Loeb extends $\cM$. The following theorem gives a necessary condition that $\cN$ contains an internal subspace which is Loeb equivalent to $\cM$. 

\begin{theorem}\label{loebnecessary}
Suppose $\cN=(\Omega, \cG, \nu)$ has an internal subspace that is Loeb equivalent to $\cM=(\Omega, \cF, \mu)$. 
Then, for every $A\in \cF$, there exists $A'\in \cF$ such that $A'\subset B\subset A$ for some $B\in \cG$ and $\mu(A')\approx \mu(A)$. 
If $\cN$ is hyperfinite, then $B$ can be taken to be $\bigcup\{C\in \cG: C\subset A\}$. 
\end{theorem} 
\begin{proof} 
Let $\cN'=(\Omega, \cG', \nu')$, where $\nu'$ is the restriction of $\nu$ to $\cG'$, be an internal subspace of $\cN$ that is Loeb equivalent to $\cM$. Pick $A\in \cF$.
By \cref{loebeqlemma}, there exists $B\in \cG$ such that $B\subset A$ and $\nu(B)\approx \mu(A)$. 
By \cref{loebeqlemma} again, we know that there exists $A'\in \cF$ such that $A'\subset B$ and $\mu(A')\approx \nu(B)$. 
\end{proof} 

\cref{loebeqq1} asks whether the converse of \cref{loebnecessary} is true. We provide a counter-example below. 

%\begin{question}\label{loebeqq1}
%Suppose $\cN$ Loeb extends $\cM$. Must $\cN$ has an internal subspace that is Loeb equivalent to $\cM$? What if $\cM$ is assumed to be hyperfinite? 
%\end{question} 
%
%The following elementary example shows that the answer to \cref{loebeqq1} is negative. 

\begin{example}\label{example1}
Let $N=\frac{1}{K!}$ for some $K\in \NSE{\Nats}\setminus \Nats$ and let $\Omega=\{\frac{1}{N}, \frac{2}{N}, \dotsc, 1\}$.
Then $\Omega$ includes the set of all rational numbers in $[0, 1]$ as a subset. 
Let $P$ denote the uniform hyperfinite probability measure on $\Omega$, that is, $P(\{\omega\})=\frac{1}{N}$ for every $\omega\in \Omega$. 
Let 
\begin{align*}
\cF=\{\emptyset, \Omega, \{\frac{1}{N}, \frac{2}{N},\dotsc, \frac{1}{2}\}, \{\frac{1}{2}+\frac{1}{N}, \dotsc, 1\}\}
\end{align*}
and let $\cG$ be the internal algebra generated by
\begin{align*}
\{\{\frac{1}{N},\frac{2}{N},\dotsc, \frac{1}{2}-\frac{2}{N}\}, \{\frac{1}{2}-\frac{1}{N},\frac{1}{2}, \frac{1}{2}+\frac{1}{N}\}, \{\frac{1}{2}+\frac{2}{N},\dotsc, 1\}\}.
\end{align*}
Let $\mu$ and $\nu$ be restrictions of $P$ on $\cF$ and $\cG$, respectively. Finally, let $\cM=(\Omega, \cF, \mu)$ and $\cN=(\Omega, \cG, \nu)$. By \cref{loebeqlemma}, it is clear that $\cN$ Loeb extends $\cM$. On the other hand, the Loeb $\sigma$-algebra $\Loeb{\cF}$ generated from $\cF$ is the same as $\cF$. Thus, $\Loeb{\cF}$ does not contain any element in $\{\{\frac{1}{N},\frac{2}{N},\dotsc, \frac{1}{2}-\frac{2}{N}\}, \{\frac{1}{2}-\frac{1}{N},\frac{1}{2}, \frac{1}{2}+\frac{1}{N}\}, \{\frac{1}{2}+\frac{2}{N},\dotsc, 1\}\}$, hence $\cM$ is not Loeb equivalent to any internal subset of $\cN$. 
\end{example}

Since the answer to \cref{loebeqq1} is negative, we now turn our attention to \cref{loebeqq2}. 
The following example shows that the answer to \cref{loebeqq2} is also negative. 

%\begin{question}\label{loebeqq2}
%Suppose $\cN$ Loeb extends $\cM$ and $\cN$ is hyperfinite. Must $\cM$ be Loeb equivalent to a hyperfinite probability space? 
%\end{question}
%
%\begin{question}\label{loebeqq3}
%Suppose $\cM=(\Omega, \cF, \mu)$ is Loeb equivalent to $\cN=(\Omega, \cG, \nu)$, and $\cH$ be the internal algebra generated by $\cF\cup \cG$.
%Must there be an internal probability measure $P$ on $\cH$ such that $\cM$ is Loeb equivalent to $(\Omega, \cH, P)$? What is $\cM$ and $\cN$ are assumed to be hyperfinite? 
%\end{question}
%
%We first give a counter-example to \cref{loebeqq2}.

\begin{example}\label{example2}
Let $N$ be an element of $\NSE{\Nats}\setminus \Nats$ and let $\Omega=\NSE{[0,1]}$. 
Let $\lambda$ denote the Lebesgue measure on $[0,1]$. 
Let $\cF$ be the internal algebra generated by $\NSE{[0,\frac{1}{2})}, \NSE{[\frac{1}{2}, 1]}$ and all $\{a\}$ for $a\in \NSE{[\frac{1}{2}-\frac{1}{N}, \frac{1}{2}+\frac{1}{N}]}$. 
Clearly, $\cF$ is not hyperfinite.
Moreover, a subset of $\NSE{[\frac{1}{2}-\frac{1}{N}, \frac{1}{2}+\frac{1}{N}]}$ is an element of $\cF$ if and only if it is hyperfinite. 
Let $\cG$ be the internal algebra generated by $\{\NSE{[0, \frac{1}{2}-\frac{1}{N})}, \NSE{[\frac{1}{2}-\frac{1}{N}, \frac{1}{2}+\frac{1}{N}]}, \NSE{(\frac{1}{2}+\frac{1}{N}, 1]}\}$. 
Let $\mu$ and $\nu$ be the restrictions of $\NSE{\lambda}$ on $\cF$ and $\cG$, respectively. 
Finally, let $\cM=(\Omega, \cF, \mu)$ and $\cN=(\Omega, \cG, \nu)$. 
It is clear that $\cN$ is hyperfinite and, by \cref{loebeqlemma}, $\cN$ Loeb extends $\cM$. 
Moreover, we have the following lemma: 
\begin{lemma}\label{loebhyperfinite}
For every internal set $F\in \Loeb{\cF}$,  $\Loeb{\mu}(F)=0$ if and only if $F$ is hyperfinite. 
\end{lemma} 
\begin{proof}
Pick $F\in \Loeb{\cF}$.
Clearly, if $F$ is hyperfinite, then $\Loeb{\mu}(F)=0$. 
If $\Loeb{\mu}(F)=0$, then there must exist $F'\in \cF$ such that $F\subset F'$ and $\mu(F')\approx 0$. 
By the construction of $\cF$, $F'$ must be hyperfinite.
As $F$ is internal, $F$ must be hyperfinite. 
\end{proof} 


We now show that $\cM$ is not Loeb equivalent to any hyperfinite probability space. 
Suppose not. Let $\cN'=(\Omega, \cG', P)$ be a hyperfinite probability space that is Loeb equivalent to $\cM$. 
For every $a\in \NSE{[\frac{1}{2}-\frac{1}{N}, \frac{1}{2}+\frac{1}{N}]}$, by \cref{loebeqlemma}, there exists $A_{a}\in \cG'$ such that $a\in A_{a}$ and $P(A_{a})\approx 0$. 
Pick $n\in \Nats$ and let 
\begin{align*}
\cA_{n}=\{A\in \cG': (P(A)<\frac{1}{n})\wedge (a\in A\ \text{for *infinitely many}\ a\in \NSE{[\frac{1}{2}-\frac{1}{N}, \frac{1}{2}+\frac{1}{N}]})\}
\end{align*}
Note that there are *infinitely many $a\in \NSE{[\frac{1}{2}-\frac{1}{N}, \frac{1}{2}+\frac{1}{N}]}$ and hyperfinitely many $A\in \cG'$ with $P(A)<\frac{1}{n}$. As each $a\in \NSE{[\frac{1}{2}-\frac{1}{N}, \frac{1}{2}+\frac{1}{N}]}$ must be contained in some $A\in \cG'$ such that $P(A)<\frac{1}{n}$, by the transfer of the pigeonhole principle, $\cA_{n}$ is non-empty for every $n\in \Nats$. 
By the saturation principle, there exists an internal $A_0$ such that $P(A_0)\approx 0$ and $A_0$ contains *infinitely many $a\in \NSE{[\frac{1}{2}-\frac{1}{N}, \frac{1}{2}+\frac{1}{N}]}$. 
As $\cN'$ is Loeb equivalent to $\cM$, we know that $\Loeb{\mu}(A_0)=0$. 
This, however, contradicts \cref{loebhyperfinite}, hence we conclude that $\cM$ is not Loeb equivalent to any hyperfinite probability space. 
\end{example}

In summary, both \cref{loebeqq1} and \cref{loebeqq2} have negative answers. 
In general, if $\cN$ Loeb extends $\cM$, it does not imply $\cM$ is equivalent to some subset of $\cN$. 



\section{Partial Solution to the Third Question}
In this section, we give a partial answer to \cref{loebeqq3}. In particular, we reduce \cref{loebeqq3} to the following question: for hyperfinite spaces, is the internal algebra generated by the union of two Loeb equivalent internal algebras a subset of the Loeb extension of any one of the internal algebra? 

Let $(\Omega, \cF, \mu)$ be an internal probability space and let $\cG$ be another internal algebra on $\Omega$. The following theorem shows that it is possible to define an internal measure $\nu$ on $(\Omega, \cG)$ such that $(\Omega, \cF, \mu)$ Loeb extends $(\Omega, \cG, \nu)$ if and only if $\cG\subset \Loeb{\cF}$.


\begin{theorem}\label{newext}
Suppose $\cM=(\Omega, \cF, \mu)$ be a hyperfinite probability space and let $\cG$ be a hyperfinite algebra on $\Omega$.
Then $(\Omega, \cF, \mu)$ Loeb extends $(\Omega, \cG, P)$ for some internal probability measure $P$ if and only if $\cG\subset \Loeb{\cF}$.  
\end{theorem}

\begin{proof}
Suppose, for some internal probability measure $P$, $(\Omega, \cF, \mu)$ Loeb extends $(\Omega, \cG, P)$. 
Then we have $\Loeb{\cG}\subset \Loeb{\cF}$ which implies that $\cG\subset \Loeb{\cF}$. 

Now suppose $\cG\subset \Loeb{\cF}$. 
As $\cF$ is hyperfinite, by the transfer principle, there exists an internal subset $\cF_0$ of $\cF$ such that
\begin{enumerate}
\item $\cF_0$ is a $\NSE{}$partition of $\Omega$
\item For every $A\in \cF_0$, if there exists non-empty $E\in \cF$ such that $E\subset A$, then $E=A$.
\end{enumerate}
Then, for any $F\in \cF$, it is a hyperfinite union of elements from $\cF_0$. Thus, $\cF_0$ generates the internal algebra $\cF$. 
Similarly, there exists an internal subset $\cG_0$ of $\cG$ such that
\begin{enumerate}
\item $\cG_0$ is a $\NSE{}$partition of $\Omega$
\item For every $A\in \cG_0$, if there exists non-empty $E\in \cG$ such that $E\subset A$, then $E=A$.
\end{enumerate}
Let $\cU=\{A\cap B: A\in \cF_0, B\in \cG_0, A\cap B\neq \emptyset\}$. 
It is easy to see that $\cU$ forms a $\NSE{}$partition of $\Omega$ and every element in $\cF\cup \cG$ can be written as a hyperfinite union of elements in $\cU$. For $F\in \cF_0$, let $\cU_{F}=\{F\cap B: B\in \cG_0, B\cap F\neq \emptyset\}$. Then $\cU=\bigcup_{F\in \cF_0}\cU_{F}$ and $\cU_{F}$ is hyperfinite for every $F\in \cF_0$. We now define a function $P': \cU\to \NSE{[0,1]}$. For every $U\in \cU$, $U\in \cU_{F_0}$ for exactly one $F_0\in \cF_0$, let $P'(U)=\frac{\mu(F_0)}{|\cU_{F_0}|}$ where $|\cU_{F_0}|$ denotes the internal cardinality of $\cU_{F_0}$. 
\begin{claim}\label{keyclaim}
For every $A\in \cF$, $\mu(A)=\sum_{U\in \cU, U\subset A}P'(U)$.
\end{claim}
\begin{proof} 
Pick $A\in \cF$. 
Let $\cF_{A}=\{F\in \cF_0: F\subset A\}$. 
For every $U\in \cU$ such that $U\subset A$, it is an element of exactly one element in $\cF_{A}$. 
Moreover, as $\cU$ forms a $\NSE{}$partition of $\Omega$, an element in $\cU$ is either a subset of $A$ or disjoint from $A$. 
Thus, we have 
\begin{align*}
\mu(A)=\sum_{F\in \cF_{A}}\mu(F)=\sum_{F\in \cF_{A}}\sum_{U\in \cU, U\subset F}\frac{\mu(F)}{|\cU_{F}|}=\sum_{U\in \cU, U\subset A}P'(U).
\end{align*}
\end{proof}

Define $P: \cG\to \NSE{[0,1]}$ by letting $P(G)=\sum_{U\in \cU, U\subset G}P'(U)$. 
\begin{claim} 
$P$ is an internal probability measure on $(\Omega, \cG)$.
\end{claim}
\begin{proof}
Clearly we have $P(\emptyset)=0$ and $P(\Omega)=1$. 
Let $G_1, G_2\in \cG$ be two disjoint sets. 
Let $U_0\subset G_1\cup G_2$ be an element of $\cU$. 
As $\cU$ forms a $\NSE{}$partition of $\Omega$ and both $G_1$ and $G_2$ can be written as a hyperfinite union of elements in $\cU$, 
we can conclude that $U_0$ is either a subset of $G_1$ or a subset of $G_2$. 
Thus, we have 
\[
P(G_1\cup G_2)&=\sum_{U\in \cU, U\subset G_1\cup G_2}P'(U)\\
&=\sum_{V\in \cU, V\subset G_1}P'(V)+\sum_{E\in \cU, E\subset G_2}P'(E)\\
&=P(G_1)+P(G_2). 
\]
\end{proof}

We now show that $(\Omega, \cF, \mu)$ Loeb extends $(\Omega, \cG, P)$. 
Pick $G\in \cG$. Let $G_i=\bigcup\{F\in \cF: F\subset G\}$ and let $G_o=\bigcap\{F\in \cF: G\subset F\}$. 
As $\cF$ is hyperfinite, both $G_i$ and $G_o$ are elements of $\cF$. 
Moreover, as $\cG\subset \Loeb{\cF}$, we have $\mu(G_i)\approx \mu(G_o)$, which implies that $\Loeb{\mu}(G)=\ST(\mu(G_i))$. 
As $G_i\subset G\subset G_o$, we have $\sum_{U\in \cU, U\subset G_i}P'(U)\leq P(G)\leq \sum_{U\in \cU, U\subset G_o}P'(U)$.
By \cref{keyclaim}, we have $\sum_{U\in \cU, U\subset G_i}P'(U)=\mu(G_i)$ and $\sum_{U\in \cU, U\subset G_o}P'(U)=\mu(G_o)$.
Thus, we can conclude that $\Loeb{P}(G)=\ST(P(G))=\ST(\mu(G_i))=\Loeb{\mu}(G)$, completing the proof. 
\end{proof}

The following theorem gives a partial answer to \cref{loebeqq3}. 

\begin{theorem}\label{unioneq}
Let $(\Omega, \cF, \mu)$ be a hyperfinite probability space and let $\cG$ be a hyperfinite algebra on $\Omega$. 
Let $\cH$ be the internal algebra generated by $\cF\cup \cG$. 
Then $(\Omega, \cH, P)$ is Loeb equivalent to $(\Omega, \cF, \mu)$ for some internal probability measure $P$ if and only if $\cH\subset \Loeb{\cF}$. 
\end{theorem}
\begin{proof} 
Suppose there exists an internal probability measure $P$ such that $(\Omega, \cH, P)$ is Loeb equivalent to $(\Omega, \cF, \mu)$. 
Then we have $\Loeb{\cH}=\Loeb{\cF}$ which implies that $\cH\subset \Loeb{\cF}$. 

Now suppose $\cH\subset \Loeb{\cF}$. 
By \cref{newext}, there exists an internal probability measure $P$ on $(\Omega, \cH)$ such that $(\Omega, \cF, \mu)$ Loeb extends 
$(\Omega, \cH, P)$. Thus, we have $P(F)\approx \mu(F)$ for every $F\in \cF$. By \cref{loebeqlemma}, $(\Omega, \cH, P)$ Loeb extends $(\Omega, \cF, \mu)$ and we have the desired result. 
\end{proof}

It is natural to ask if \cref{unioneq} remains valid without the hyperfinite assumption. 
\begin{open problem}
Let $\cM=(\Omega, \cF, \mu)$ and $\cN=(\Omega, \cG, \nu)$ be two internal probability spaces that are not hyperfinite.
Let $\cH$ be the internal algebra generated by $\cF\cup \cG$.
Suppose $\cM$ is Loeb equivalent to $\cN$, and $\cH\subset \Loeb{\cF}$.
Must there be an internal probability measure $P$ on $\cH$ such that $\cM$ is Loeb equivalent to $(\Omega, \cH, P)$?
\end{open problem}




\section{Loeb Measurability of $\cH$}
We have shown in previous section that \cref{loebeqq3} is equivalent to the following fundamental problem in Loeb measure theory:
\begin{open problem}\label{posloebquestion}
Let $(\Omega, \cF, \mu)$ be a hyperfinite probability space and let $\cG$ be another hyperfinite algebra on $\Omega$ such that $\cG\subset \Loeb{\cF}$. Let $\cH$ be the hyperfinite algebra generated by $\cF\cup \cG$. Is $\cH\subset \Loeb{\cF}$? 
\end{open problem}
We suspect the answer to \cref{posloebquestion} is negative. However, in this section, we provide a few sufficient conditions that lead to positive answer to \cref{posloebquestion}. 
Let $\cM=(\Omega, \cF, \mu)$ and $\cN=\{\Omega, \cG, \nu\}$ be two hyperfinite probability spaces.
We use the same notation as in the proof of \cref{newext} 
Throughout this section, let $\cF_0$ be an internal subset of $\cF$ such that 
\begin{enumerate}
\item $\cF_0$ is a $\NSE{}$partition of $\Omega$
\item For every $A\in \cF_0$, if there exists non-empty $E\in \cF$ such that $E\subset A$, then $E=A$.
\end{enumerate}
Similarly, let $\cG_0$ be an internal subset of $\cG$ such that
\begin{enumerate}
\item $\cG_0$ is a $\NSE{}$partition of $\Omega$
\item For every $A\in \cG_0$, if there exists non-empty $E\in \cG$ such that $E\subset A$, then $E=A$.
\end{enumerate}
Let $\cU=\{A\cap B: A\in \cF_0, B\in \cG_0, A\cap B\neq \emptyset\}$. Then $\cU$ forms a $\NSE{}$partition of $\Omega$ and every element in $\cH$ can be written as a hyperfinite union of elements in $\cU$. It follows from the Loeb measurability of $\cG$ that $\cU\subset \Loeb{\cF}$. However, it is not clear whether all hyperfinite (not finite) unions of elements in $\cU$ is an element of $\Loeb{\cF}$. Hence it is not straightforward to determine the Loeb measurability of $\cH$. Finally, let $\cF_0'=\{F\in \cF_0: \text{$F$ intersects at least two elements in $\cG_0$}\}$. 

\begin{theorem}\label{immthm}
Suppose $\cG\subset \Loeb{\cF}$ and $\mu(\bigcup \cF_0')\approx 0$. 
Then $\cH\subset \Loeb{\cF}$. 
\end{theorem}
\begin{proof} 
Let $\cF_1=\cF_0\setminus \cF_0'$. 
Pick $H\in \cH$ and, without loss of generality, assume that $H=\bigcup_{i=1}^{K}(A_i\cap B_i)$ where $A_i\in \cF$, $B_i\in \cG$ and $K\in \NSE{\Nats}$.
Let $\cV=\{A_i\cap B_i: i\leq K\}$. 
Then $H=H_1\cup H_2$ where $H_1=\bigcup \{(A_i\cap B_i)\in \cV: A_i\in \cF_0'\}$ and $H_2=\bigcup \{(A_i\cap B_i)\in \cV: A_i\in \cF_1\}$. 
Clearly, $H_1$ is a subset of $\bigcup \cF_0'$. 
As $\mu(\bigcup \cF_0')\approx 0$, by the completeness of Loeb measure, $H_1$ is Loeb measurable and $\Loeb{\mu}(H_1)=0$.
Note that, for every element $F\in \cF_1$, there exists an unique $G\in \cG_0$ such that $F\subset G$. 
Thus, for every $A_i\in \cF_1$, $A_i\cap B_i$ is either $A_i$ or $\emptyset$.
Thus, we know that $H_2\in \cF$.
Hence we conclude that $H\in \Loeb{\cF}$, completing the proof. 
\end{proof} 

We now explore some sufficient conditions that would imply $\mu(\bigcup \cF_0')\approx 0$. We start with the following lemma. 

\begin{lemma}\label{loebseparate}
Let $(\Omega, \cF, \mu)$ be a hyperfinite probability space and let $\cG$ be a hyperfinite algebra on $\Omega$ such that $\cG\subset \Loeb{\cF}$.
Let $\cA$ be an internal subset of $\cF_0'$. 
Suppose there exists $G_1\in \cG$ such that both $G_1$ and $\Omega\setminus G_1$ intersects every element in $\cA$. 
Then $\mu(\bigcup \cA)\approx 0$.  
\end{lemma}
\begin{proof} 
Let $F_{G_1}=\bigcap\{F\in \cF: G_1\subset F\}$. 
Since $G_1$ intersects every element in $\cA$, we know that $\bigcup \cA\subset F_{G_1}$. 
Thus, by the Loeb measurability of $G_1$, we know that $\bigcup \cA\setminus G_1$ has Loeb measure $0$. 
Similarly, we can conclude that $\bigcup \cA\setminus (\Omega\setminus G_1)$ has Loeb measure $0$. 
Thus, we can conclude that $\mu(\bigcup \cA)\approx 0$. 
\end{proof}

We now consider the collection of sets in $\cF$ with infinitesimal measure. 
We show that, if for every $F\in \cF$ with $\mu(F)\approx 0$, there exists some $G\in \cG_0$ such that $F\cap G=\emptyset$, 
then $\mu(\bigcup \cF_0')\approx 0$, which, by \cref{immthm}, implies that $\cH\subset \Loeb{\cF}$ (see \cref{measurecor}).
We start with the following technical lemma. 

\begin{lemma}\label{measureapproach}
Let $(\Omega, \cF, \mu)$ be an internal probability measure and let $\cG$ be an internal algebra on $\Omega$ such that $\cG\subset \Loeb{\cF}$.
Let $\cI_0\subset \cF$ consist of all sets $A$ such that: 
\begin{enumerate}
\item $\mu(A)\approx 0$
\item For all $G\in \cG_0$, $A\cap G\neq \emptyset$. 
\item For all $B\in \cF$ such that $B$ is a proper subset of $A$, there exists some $G\in \cG_0$ such that $B\cap G=\emptyset$.
\end{enumerate}
Then $\bigcup \cI_0$ is $\Loeb{\mu}$-measurable
and $\Loeb{\mu}(\bigcup \cF_0'\setminus \bigcup \cI_0)=0$.
\end{lemma}

\begin{proof}
For $n\in \Nats$, let $\cI_n\subset \cF$ consist of all sets $A$ such that: 
\begin{enumerate}
\item $\mu(A)\leq \frac{1}{n}$
\item For all $G\in \cG_0$, $A\cap G\neq \emptyset$. 
\item For all $B\in \cF$ such that $B$ is a proper subset of $A$, there exists some $G\in \cG_0$ such that $B\cap G=\emptyset$.
\end{enumerate}
By the internal definition principle, $\cI_n$ is internal for every $n\in \Nats$. 
As $\cF$ is hyperfinite, we have $\bigcup \cI_n\in \cF$ for every $n\in \Nats$. 
As $\cI_0=\bigcap_{n\in \Nats} \cI_n$, we conclude that $\bigcup \cI_0=\bigcap_{n\in \Nats}\bigcup \cI_n$ is $\Loeb{\mu}$-measurable. 

Suppose $\Loeb{\mu}(\bigcup \cF_0'\setminus \bigcup \cI_0)>0$.
Let $\cJ_0=\{F\in \cF_0': (\exists A\in \cI_0)(F\subset A)\}$. 
It is easy to see that $\bigcup \cJ_0\subset\bigcup \cI_0$. 
Let $\cE$ be the internal algebra generated by $\cC=\cF_0'\setminus \cJ_0$. 
We immediately have $\Loeb{\mu}(\bigcup \cC)>0$.
%Let 
%\[
%\cV=\{r\in \NSE{\Reals}: (\text{There exists an internal $\cD\subset \cC$ with $\mu(\bigcup \cD)\geq r$})\phi(\cD)\}
%\]
%where $\phi(\cD)$ is the formula $(\exists G\in \cG)\ (\text{$G$ and $\Omega\setminus G$ intersect every element in $\cD$})$.
We now consider the following algorithm. 
\begin{enumerate}
\item Pick any element $G_1\in \cG_0$ and let $\cC_{G_1}=\{C\in \cC: C\cap G_1\neq \emptyset\}$.

\item For $k\geq 2$, assuming $G_1,\dotsc, G_{k-1}$ have already been chosen, pick $G_k\in \cG_0$ such that 
$G_k\cap \bigcup_{i=1}^{k-1}\bigcup \cC_{G_i}=\emptyset$. 
\end{enumerate}
We continue this process until we reach a natural stopping point. 
Without loss of generality, we assume that this algorithm continue for $K\in \NSE{\Nats}$ many steps 
and consider the set $\bigcup_{i=1}^{K}\bigcup \cC_{G_i}$. 
By construction, for every $A\in \cE$ such that $\mu(A)\approx 0$, there exists some $G\in \cG_0$ such that $B\cap G=\emptyset$.
Hence, we can conclude that $\Loeb{\mu}(\bigcup_{i=1}^{K}\bigcup \cC_{G_i})>0$. 
By construction, both $\bigcup_{i=1}^{K} G_i$ and its complement intersect every element in $\bigcup_{i=1}^{K}\bigcup \cC_{G_i}$. 
By \cref{loebseparate}, this is a contradiction. 
\end{proof}

An immediate consequence of \cref{measureapproach} is:

\begin{lemma}\label{resultmeasure}
Let $(\Omega, \cF, \mu)$ be an internal probability measure and let $\cG$ be an internal algebra on $\Omega$ such that $\cG\subset \Loeb{\cF}$. Let $\cF_0$ and $\cG_0$ be the collections of atoms as defined in the beginning of the section. 
%Let $\cF_0'=\{F\in \cF_0: \text{$F$ intersect with at least two elements in $\cG_0$}\}$.
Let $\cI_0$ be the same set as in the statement of \cref{measureapproach}. 
Suppose $\Loeb{\mu}(\bigcup \cI_0)=0$. 
Then $\cH\subset \Loeb{\cF}$. 
\end{lemma}
\begin{proof}
By \cref{measureapproach} and the fact that $\Loeb{\mu}(\bigcup \cI_0)=0$, we can conclude that $\Loeb{\mu}(\bigcup \cF_0')=0$. 
By \cref{immthm}, $\cH\subset \Loeb{\cF}$. 
\end{proof}

We now present the main result of this section, which follows immediately from \cref{resultmeasure}: 

\begin{theorem}\label{measurecor}
Let $(\Omega, \cF, \mu)$ be an internal probability measure and let $\cG$ be an internal algebra on $\Omega$ such that $\cG\subset \Loeb{\cF}$. Let $\cF_0$ and $\cG_0$ be the collections of atoms as defined in the beginning of the section. 
Suppose, for every $F\in \cF$ with $\mu(F)\approx 0$, there exists $G\in \cG_0$ such that $F\cap G=\emptyset$. 
Then $\cH\subset \Loeb{\cF}$. 
\end{theorem}
\begin{proof}
By the assumption of the theorem, we know that $\cI_0$ is empty. 
The result then follows from \cref{resultmeasure}.
\end{proof}

\cref{measurecor} provides a quick way to identify the Loeb measurability of $\cH$. We conclude with the following open question. 

\begin{open problem}
Let $\cM=(\Omega, \cF, \mu)$ and $\cN=(\Omega, \cG, \nu)$ be two hyperfinite probability spaces. 
If $\Loeb{\mu}(\bigcup \cF_0')>0$, is it possible that $\cH\subset \Loeb{\cF}$? 
\end{open problem}

%In conclusion, if $\bigcup F_0'$ is a Loeb null set, then we have a positive answer for \cref{posloebquestion}. The next theorem, however, shows that it is not always the case. 
%
%\begin{theorem}\label{poscounter}
%Let $\Omega=\NSE{[0,1]}$ and $K\in \NSE{\Nats}\setminus \Nats$. 
%Let $\cF_0=\{[0, \frac{1}{N}), [\frac{1}{N},\frac{2}{N}),\dotsc,[\frac{N-1}{N}, 1]\}$ and let $\cF$ be the  algebra generated by $\cF_0$. Let $\mu$ be an internal probability measure on $(\Omega, \cF)$ such that $\mu(A)=\frac{1}{N}$. Then there exists a hyperfinite algebra $\cG$ on $\Omega$ such that 
%\begin{enumerate}
%\item $\cG$ is generated by some set of atoms $\cG_0$
%
%\item $\cG\subset \Loeb{\cF}$ 
%
%\item $\Loeb{\mu}(\bigcup \cF_0(\cG))>0$, where $\cF_0(\cG)=\{F\in \cF_0: \text{$F$ intersect with at least two elements in $\cG_0$}\}$.
%\end{enumerate}
%\end{theorem}
%\begin{proof}
%Note that every hyperfinite algebra is generated by some set of atoms. 
%Thus, the first condition is satisfied automatically. 
%
%
%
%
%
%
%
%
%
%
%
%\end{proof}

%\section{Bob's approach}
%
%\begin{theorem}
%Let $X$ be a hyperfinite set and let $P$ be an internal probability measure on the internal power set $\NSE{\PowerSet(X)}$ of $X$. 
%Let $\cF$ and $\cG$ be two internal algebras such that $\Loeb{\cF}\supset \Loeb{\cG}$. 
%Let $\cH$ be the internal algebra generated by $\cF\cup \cG$. 
%Then, for every set $H\in \cH$, there exists $F_{H}\in \cF$ such that $P(H\symdiff F_{H})\approx 0$. 
%\end{theorem}
%
%\begin{proof}
%Let $\cF_0$ and $\cG_0$ be the collection of ``atoms" that generate $\cF$ and $\cG$, respectively. 
%Then, $\cH$ is generated by $\cH_0=\{F\cap G: F\in \cF_0, G\in \cG_0, F\cap G\neq \emptyset\}$. 
%For $n\in \Nats$, let 
%\[
%\cF_n=\{F\in \cF_0: (\exists B\in \cG)(\frac{1}{n}<\frac{P(F\cap B)}{P(F)}<1-\frac{1}{n})\}.
%\]
%By the internal definition definition principle, $\bigcup \cF_n$ is an element of $\cF$. 
%For each $F\in \cF_n$, pick $D_{F}^{n}\in \cG$ such that $\frac{1}{n}<\frac{P(F\cap D_{F}^{n})}{P(F)}<1-\frac{1}{n}$. 
%Let $D_n=\bigcup_{F\in \cF_n}D_{F}^{n}$. It is easy to see that $D_n\in \cG$. 
%Let $C=\bigcup_{n\in \Nats}\bigcup \cF_n$. Then $C\in \Loeb{\cF}$. Moreover, $\Loeb{P}(C)>0$ if and only if $\Loeb{P}(\bigcup \cF_n)>0$ for some $n\in \Nats$. 
%
%Suppose $\Loeb{P}(C)>0$. Pick $n\in \Nats$ such that $P(\bigcup \cF_n)>\frac{1}{m}$ for some $m\in \Nats$. 
%Let $E\in \cF$ be a subset of $D_n$. 
%Then, for every $F\in \cF_n$, we have $\frac{P(F\cap E)}{P(F)}\leq \frac{P(F\cap D_n)}{P(F)}<1-\frac{1}{n}$. 
%Thus, we conclude that $E\cap \bigcup \cF_n=\emptyset$. 
%Therefore, we have $P(D_n\setminus E)>P(D_{F}^{n}\setminus E)>P(F\cap D_{F}^{n})>\frac{1}{nm}$. 
%Thus, $D_n$ is not an element of $\Loeb{\cF}$ so we conclude that $\Loeb{P}(C)=0$. 
%
%Now consider an arbitrary element $H\in \cH$.
%It is easy to see that $H=\bigcup_{i=1}^{K} (I_i\cap J_i)$ where $I_i\cap J_i\in \cH_0$ and $K\in \NSE{\Nats}$. 
%Let $H_1=\{I_i: I_i\in \bigcup_{n\in \Nats}\cF_n\}$. 
%As $\Loeb{P}(C)=0$, by the completeness of Loeb measure, we conclude that $\Loeb{P}(\bigcup_{I_i\in H_1}I_i\cap J_i)=0$. 
%Let $H_2=\{I_i: \frac{P(I_i\cap J_i)}{P(I_i)}\approx 0\}$ and $H_3=\{I_i: \frac{P(I_i\cap J_i)}{P(I_i)}\approx 1\}$. 
%
%\begin{claim}\label{Hclaim}
%Both $\bigcup_{I_i\in H_2}I_i\cap J_i$ and $\bigcup_{I_i\in H_3}I_i\cap J_i$ are elements of $\Loeb{\NSE{\PowerSet(X)}}$. 
%Moreover, $\Loeb{P}(\bigcup_{I_i\in H_3}I_i\symdiff H)= 0$. 
%\end{claim}
%\begin{proof}
%For $n\in \Nats$, let $H_2^{(n)}=\{I_i: \frac{P(I_i\cap J_i)}{P(I_i)}<\frac{1}{n}\}$ 
%and $H_3^{(n)}=\{I_i: \frac{P(I_i\cap J_i)}{P(I_i)}>1-\frac{1}{n}\}$. 
%Then $H_2=\bigcap_{n\in \Nats}H_2^{(n)}$ and $H_3=\bigcap_{n\in \Nats}H_3^{(n)}$. 
%Thus, both $\bigcup_{I_i\in H_2}I_i\cap J_i$ and $\bigcup_{I_i\in H_3}I_i\cap J_i$ are elements of $\Loeb{\NSE{\PowerSet(X)}}$. 
%
%For every $n\in \Nats$, we have 
%\[
%P(\bigcup_{I_i\in H_2^{(n)}}I_i\cap J_i)<\frac{1}{n}P(\bigcup_{I_i\in H_2^{(n)}}I_i)\leq \frac{1}{n}. 
%\]
%Hence we know that $\Loeb{P}(\bigcup_{I_i\in H_2}I_i\cap J_i)=0$. 
%Similarly, we know that $\Loeb{P}(\bigcup_{I_i\in H_3}(I_i\setminus J_i)=0$. 
%Thus, $\bigcup_{I_i\in H_3}I_i$ and $\bigcup_{I_i\in H_3}I_i\cap J_i$ have the same Loeb measure. 
%As $\Loeb{P}(\bigcup_{I_i\in H_2}I_i\cap J_i)=0$ and $\Loeb{P}(\bigcup_{I_i\in H_1}I_i\cap J_i)=0$, 
%we know that $\Loeb{P}(\bigcup_{I_i\in H_3}I_i\symdiff H)=0$
%\end{proof}
%
%As $\bigcup_{I_i\in H_3}I_i$ is an element of $\Loeb{\cF}$, there exists $F_{H}\in \cF$ such that 
%$\Loeb{P}(F_{H}\symdiff \bigcup_{I_i\in H_3}I_i)=0$.
%By \cref{Hclaim}, we know that $P(H\symdiff F_{H})\approx 0$. 
%\end{proof}



%\section{old stuff}
%
%
%\begin{definition}\label{cmnsreal}
%Let $r_1, r_2$ be two nonzero elements of $\NSE{\Reals}$. 
%\begin{itemize}
%\item We say $r_1$ is relatively large to $r_2$ (and write $r_1\rbig r_2$) if $\frac{|r_1|}{|r_2|}>n$ for every $n\in \Nats$.
%\item We say $r_1$ is relatively equal to $r_2$ (and write $r_1\requal r_2$) if $\frac{|r_1|}{|r_2|}\approx r$ for some positive $r\in \Reals$.
%\item We say $r_1$ is relatively small to $r_2$ (and write $r_1\rsmall r_2$) if $\frac{|r_1|}{|r_2|}<\frac{1}{n}$ for every $n\in \Nats$.
%\end{itemize}
%\end{definition}
%Clearly, $r_1$ is relatively large to $r_2$ if and only if $r_2$ is relatively small to $r_1$. The following definitions are crucial to our main result in this section. 
%
%\begin{definition}\label{defuni}
%Let $(\Omega, \cF, \mu)$ be a hyperfinite probability space and let $\cF_0$ be defined as in the beginning of this section. 
%$(\Omega, \cF, \mu)$ is said to be \textbf{quasi uniform} if there exists $K\in \NSE{\Nats}$ such that, for any internal $\cA\subset \cF_0$, 
%$\Loeb{\mu}(\bigcup \cA)=0$ if and only if $|\cA|\rsmall K$.
%\end{definition}
%For a quasi uniform hyperfinite probability space $(\Omega, \cF, \mu)$, it is easy to see that $K\requal |\cF_0|$. 
%
%\begin{definition}\label{redensity}
%Let $(\Omega, \cF, \mu)$ be a hyperfinite probability space and let $\cG$ be a hyperfinite algebra on $\Omega$. 
%Let $\cA$ be an internal subset of $\cG$. 
%For every $F\in \cF$, define $\des{\cA}{F}=|\{G\in \cA: G\cap F\neq \emptyset\}|$. 
%We call $\des{\cA}{F}$ \textbf{the relative density of $F$ with respect to $\cA$}. 
%\end{definition}
%
%We now present the main technical result of this section. 
%
%\begin{lemma}\label{maintechnical}
%Let $(\Omega, \cF, \mu)$ be a quasi uniform hyperfinite probability space and $\cG$ be a hyperfinite algebra on $\Omega$ such that $\cG\subset \Loeb{\cF}$.
%Let $\cF_0$ and $\cG_0$ be defined as in the beginning of the section. 
%Let $\cF_0'=\{F\in \cF_0: \text{$F$ intersect with at least two elements in $\cG_0$}\}$ 
%and $\cG_0'=\{G\in \cG_0: (\exists F\in \cF_0')(G\cap F\neq \emptyset)\}$. 
%Suppose $|\cF_0|\requal |\cG_0|$ and $\des{\cG_0}{F}$ is finite for every $F\in \cF_0$.
%Then $\mu(\bigcup \cF_0')\approx 0$. 
%\end{lemma}
%\begin{proof}
%By the construction of $\cF_0'$, we know that $|\cG_0\setminus \cG_0'|\leq |\cF_0\setminus \cF_0'|$. 
%As $|\cF_0|\requal |\cG_0|$, we know that either $|\cF_0'|\requal |\cG_0'|$ or $|\cF_0'|\rsmall |\cG_0'|$. 
%Suppose $\Loeb{\mu}(\bigcup \cF_0')>0$. 
%By the quasi uniformity of $(\Omega,\cF,\mu)$, we know that $|\cF_0'|\requal |\cF_0|\requal |\cG_0'|$. 
%%\begin{claim}\label{claim1}
%%For every $n\in \Nats$, $\Loeb{\mu}(\bigcup \cF_n')=0$ where $\cF_n'=\{F\in \cF_0': \des{\cG_0'}{F}>\frac{1}{n} |\cG_0'|\}$. 
%%\end{claim}
%%\begin{proof}
%%Suppose not. Then there exists some $n\in \Nats$ such that $\Loeb{\mu}(\bigcup \cF_n')>0$. 
%%By the uniformity of $(\Omega, \cF, \mu)$, we know that $|\cF_n'|\requal |\cF_0'|\requal |\cF_0|$. 
%%We now consider the set 
%%\[
%%\cL=\{N\in \NSE{\Nats}: (\text{For all internal $\cA\subset \cF_n'$ with $|\cA|\leq N$})\phi(\cA)\},
%%\]
%%where $\phi(\cA)$ is the formula $(\exists G\in \cG_0')\ (\text{$G$ and $\Omega\setminus G$ intersect every element in $\cA$})$.
%%We now show that $\cL$ contains all $N\rsmall |\cF_n'|$. 
%%Pick an arbitrary internal $\cA_0\subset \cF_n'$ with $|\cA_0|\rsmall |\cF_n'|$.
%%For each element $A\in \cA_0$, pick $G_{A}\in \cG_0'$ such that $G_A\cap A\neq \emptyset$. 
%%Clearly, $\bigcup_{A\in \cA_0}G_{A}$ intersect with every element in $\cA_0$. 
%%On the other hand, as $\des{\cG_0'}{A}>\frac{1}{n} |\cG_0'|$ for every $A\in \cA_0$, 
%%we know that $\Omega\setminus (\bigcup_{A\in \cA_0}G_{A}$ intersect with every element in $\cA_0$. 
%%Hence, we can conclude that $\cL$ contains all $N\rsmall |\cF_n'|$. 
%%As $\cL$ is an internal set, by overspill, it must contain some $N_0\requal |\cF_n'|$. 
%%That is, there exists an internal $\cA_1\subset \cF_n'$ with $|\cA_1|\requal |\cF_n'|$ such that $\phi(\cA_1)$ holds. 
%%By the uniformity of $(\Omega, \cF, \mu)$, we know that $\Loeb{\mu}(\bigcup \cA_1)>0$. 
%%By \cref{loebseparate}, we have a contradiction.  
%%\end{proof}
%%By \cref{claim1} and overspill ,the set $\{n\in \NSE{\Nats}: \mu(\bigcup \cF_n')<\frac{1}{n}\}$ contains some infinite $N\in \NSE{\Nats}$. 
%%That is, we have $\Loeb{\mu}(\bigcup\cF_{N}')=0$. We now consider the set 
%%\[
%%\cE_0'=\{F\in \cF_0': \des{\cG_0'}{F}\leq \frac{1}{N} |\cG_0'|\}=\cF_0'\setminus \cF_{N}'.
%%\] 
%%
%%
%%\begin{claim}\label{claim2}
%%The set $\bigcup\cE_0'$ has Loeb measure $0$. 
%%\end{claim}
%%\begin{proof} 
%We now consider the set 
%\[
%\cI=\{N\in \NSE{\Nats}: (\text{There exists an internal $\cA\subset \cF_0'$ with $|\cA|\geq N$})\phi(\cA)\}
%\]
%where $\phi(\cA)$ is the formula $(\exists G\in \cG_0')\ (\text{$G$ and $\Omega\setminus G$ intersect every element in $\cA$})$.
%We now show that $\cI$ contains all $N\rsmall |\cF_0'|$ by introducing the following algorithm. 
%\begin{enumerate}
%\item Pick any element $G_1\in \cG_0'$ and let $\cF_{G_1}=\{F\in \cF_0': F\cap G_1\neq \emptyset\}$.
%
%\item For $k\geq 2$, suppose $G_1,\dotsc, G_{k-1}$ have already been chosen, pick $G_k\in \cG_0'$ such that 
%$G_k\cap \bigcup_{i=1}^{k-1}\bigcup \cF_{G_i}=\emptyset$. 
%\end{enumerate}
%For every $G\in \cV$, by \cref{loebseparate} and quasi uniformity, we know that $|\cF_{G}|\rsmall |\cF_0'|$.
%as $\des{\cG_0}{F}$ is finite for every $F\in \cF_0$
%As $|\cG_0'|$ is at least relatively equal to $|\cF_0'|$ and $\des{\cG_0}{F}$ is finite for every $F\in \cF_0$, the number of elements in $\cG_0'$ that intersect with $\bigcup \cF_{G}$ is relatively small to $|\cG_0'|$. That is, this algorithm would continue for any $k$ steps as long as $|\bigcup_{i=1}^{k-1}\cF_{G_i}|\rsmall |\cF_0'|$. 
%Moreover, both $\bigcup_{i=1}^{k}G_i$ and its complement intersect with every element in $\bigcup_{i=1}\cF_{G_i}$. 
%Thus, $\bigcup_{i=1}\cF_{G_i}$ is an internal subset of $\cF_0'$ such that $|\bigcup_{i=1}\cF_{G_i}|\geq N$ and $\phi(\bigcup_{i=1}\cF_{G_i})$ holds. 
%Hence, we can conclude that $\cI$ contains all $N\rsmall |\cF_0'|$. 
%By overspill, there exists an internal $\cC\subset \cF_0'$ with $|\cC|\requal |\cF_0'|$ such that $\phi(\cC)$ holds. 
%By the uniformity of $(\Omega, \cF, \mu)$ and \cref{loebseparate}, this is a contradiction. 
%Hence we have $\Loeb{\mu}(\bigcup \cF_0')=0$, completing the proof. 
%\end{proof}



\printbibliography


==> loeb equivalence arxiv/myvruler.tex <==
\usepackage{vruler}
\setvruler[10pt][1][1][4][1][20pt][20pt][0pt][\textheight]
\let\orgfillzeros\fillzeros
\def\fillzeros[#1]#2{%
  \begingroup
    \color[rgb]{0.8,0.8,0.8}%
    \orgfillzeros[{#1}]{#2}%
  \endgroup
}


==> loeb equivalence arxiv/novruler.tex <==
% nothing here


==> myvruler.tex <==
\usepackage{vruler}
\setvruler[10pt][1][1][4][1][20pt][20pt][0pt][\textheight]
\let\orgfillzeros\fillzeros
\def\fillzeros[#1]#2{%
  \begingroup
    \color[rgb]{0.8,0.8,0.8}%
    \orgfillzeros[{#1}]{#2}%
  \endgroup
}


==> novruler.tex <==
% nothing here

